Emergent Spacetime and Holographic CFTs

We discuss universal properties of conformal field theories with holographic duals. A central feature of these theories is the existence of a low-lying sector of operators whose correlators factorize. We demonstrate that factorization can only hold in the large central charge limit. Using conformal invariance and factorization we argue that these operators are naturally represented as fields in AdS as this makes the underlying linearity of the system manifest. In this class of CFTs the solution of the conformal bootstrap conditions can be naturally organized in structures which coincide with Witten diagrams in the bulk. The large value of the central charge suggests that the theory must include a large number of new operators not captured by the factorized sector. Consequently we may think of the AdS hologram as an effective representation of a small sector of the CFT, which is embedded inside a much larger Hilbert space corresponding to the black hole microstates.

==> toc.tex <==
\noindent {1.} {Introduction} \leaderfill{3} \par 
\noindent {2.} {Main Picture: conditions for holographic CFTs} \leaderfill{6} \par 
\noindent \quad{2.1.} {Some comments} \leaderfill{9} \par 
\noindent \quad{2.2.} {Examples} \leaderfill{12} \par 
\noindent \quad{2.3.} {Counter-Examples} \leaderfill{18} \par 
\noindent \quad{2.4.} {Do we need gauge-symmetry?} \leaderfill{20} \par 
\noindent {3.} {Consistency Requirements for a CFT} \leaderfill{21} \par 
\noindent \quad{3.1.} {Conformal Bootstrap} \leaderfill{22} \par 
\noindent \quad{3.2.} {Modular Invariance and consistency at finite temperature} \leaderfill{25} \par 
\noindent \quad{3.3.} {``Cardy formula'' and higher dimensional CFTs} \leaderfill{29} \par 
\noindent {4.} {Generalized Free CFTs and holography} \leaderfill{30} \par 
\noindent \quad{4.1.} {Generalized free fields: factorization for $\Delta >{d-2 \over 2}$} \leaderfill{31} \par 
\noindent \quad{4.2.} {Conformal bootstrap for generalized free fields and multiparticle spectrum} \leaderfill{32} \par 
\noindent \quad{4.3.} {Partition functions of generalized free fields} \leaderfill{34} \par 
\noindent \quad{4.4.} {Decoupling of the stress tensor and the need for large $c$} \leaderfill{37} \par 
\noindent \quad{4.5.} {Gravitational collapse and ``deconfinement''} \leaderfill{39} \par 
\noindent \quad{4.6.} {Minimal generalized free CFT and gas of gravitons} \leaderfill{42} \par 
\noindent \quad{4.7.} {Summary} \leaderfill{43} \par 
\noindent {5.} {Emergence of the holographic dimension} \leaderfill{44} \par 
\noindent \quad{5.1.} {Why this is not just group theory.} \leaderfill{46} \par 
\noindent \quad{5.2.} {Operators with spin} \leaderfill{47} \par 
\noindent \quad{5.3.} {Comments on bulk observables and background independence} \leaderfill{48} \par 
\noindent {6.} {Including interactions} \leaderfill{49} \par 
\noindent \quad{6.1.} {Scaling of Correlators with $c$} \leaderfill{50} \par 
\noindent \quad{6.2.} {Conformal bootstrap in perturbation theory and holographic interactions} \leaderfill{52} \par 
\noindent \quad{6.3.} {CFT interpretation of Witten diagrams: ``dressed'' conformal blocks} \leaderfill{54} \par 
\noindent \quad{6.4.} {Summary: CFT interpretation of the basic exchange Witten diagram} \leaderfill{59} \par 
\noindent \quad{6.5.} {Dressing the OPE} \leaderfill{60} \par 
\noindent \quad{6.6.} {Conformal bootstrap for higher $n$-point functions} \leaderfill{62} \par 
\noindent \quad{6.7.} {Generalized free CFTs and expansion in Witten diagrams} \leaderfill{65} \par 
\noindent {7.} {The CFT at finite temperature} \leaderfill{66} \par 
\noindent \quad{7.1.} {Factorization requires an infinite number of degrees of freedom} \leaderfill{67} \par 
\noindent \quad{7.2.} {Hawking-Page transition ?} \leaderfill{69} \par 
\noindent \quad{7.3.} {Extending the ``Cardy regime''?} \leaderfill{71} \par 
\noindent {8.} {Discussions} \leaderfill{72} \par 
\noindent Appendix {A.} {Conformal Partial Waves} \leaderfill{74} \par 
\noindent Appendix {B.} {CPW expansion of Witten diagrams} \leaderfill{75} \par 
\noindent \quad{\hbox {B.}1.} {Contact Witten diagram} \leaderfill{76} \par 
\noindent \quad{\hbox {B.}2.} {Exchange Witten diagram} \leaderfill{78} \par 
\noindent Appendix {C.} {Central charges in higher dimensional CFTs} \leaderfill{81} \par 

